On the Invariance of G\"odel's Second Theorem with regard to Numberings

The prevalent interpretation of G\"odel's Second Theorem states that a sufficiently adequate and consistent theory does not prove its consistency. It is however not entirely clear how to justify this informal reading, as the formulation of the underlying mathematical theorem depends on several arbitrary formalisation choices. In this paper I examine the theorem's dependency regarding G\"odel numberings. I introduce deviant numberings, yielding provability predicates satisfying L\"ob's conditions, which result in provable consistency sentences. According to the main result of this paper however, these "counterexamples" do not refute the theorem's prevalent interpretation, since once a natural class of admissible numberings is singled out, invariance is maintained.

==> Submission Arxiv/balthasar.macros.tex <==
%% Personal Macros %%%

%Nicer Phi:
\renewcommand{\phi}{\varphi}

%No rule in Epigraph:
\setlength{\epigraphrule}{0pt}

%Godel numerals:
\newbox\gnBoxA
\newdimen\gnCornerHgt
\setbox\gnBoxA=\hbox{$\ulcorner$}
\global\gnCornerHgt=\ht\gnBoxA
\newdimen\gnArgHgt
\newcommand{\gn}[2]{%
	\setbox\gnBoxA=\hbox{$#1$}%
	\gnArgHgt=\ht\gnBoxA%
	\ifnum     \gnArgHgt<\gnCornerHgt \gnArgHgt=0pt%
	\else \advance \gnArgHgt by -\gnCornerHgt%
	\fi \raise\gnArgHgt\hbox{$\ulcorner$} \box\gnBoxA %
	\raise\gnArgHgt\hbox{$\urcorner^{#2}$}}

%Concatenation Symbol:
\newcommand{\concat}{%
	\mathord{
		\mathchoice
		{\raisebox{1ex}{\scalebox{.7}{$\frown$}}}
		{\raisebox{1ex}{\scalebox{.7}{$\frown$}}}
		{\raisebox{.7ex}{\scalebox{.5}{$\frown$}}}
		{\raisebox{.7ex}{\scalebox{.5}{$\frown$}}}
	}
}

%simple quotation symbols for math mode:
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}

%for axiomatic calculus:
\newcounter{bew}
\newcommand\bwz[2]{&(\arabic{bew})&&#1&&\text{#2}\stepcounter{bew}}
\newcommand\bwzo[2]{& &&#1&&\text{#2}}%fur zeilenumbruch in nbeweis
\newenvironment{nbeweis}{\setcounter{bew}{1}\csname align*\endcsname}{\csname endalign*\endcsname}

%nicer restriction symbol:
\renewcommand{\restriction}{\mathord{\upharpoonright}}

\DeclareMathOperator{\dom}{dom} %fuer domain

%logical connectives for metalanguage
\newcommand{\Forall}{\raisebox{0.15em}{\scalebox{0.72}{$\backslash$}}\hspace{-0.18em}\forall}
\newcommand{\Exists}{\exists\hspace{-0.45em}\exists}
\newcommand{\Neg}{\neg\hspace{-0.5em}\neg}
\newcommand{\Lor}{\;\raisebox{-0.12em}{\begin{turn}{90}$\eqslantless$\end{turn}}\;}
\newcommand{\Land}{\;\raisebox{-0.12em}{\begin{turn}{90}$\eqslantgtr$\end{turn}}\;}

% hash symbol for Visser numbering:
\newcommand\hash{\mathbin{\mathpalette\xhash\relax}}
\newcommand{\xhash}[2]{\ooalign{%
		$#1\xxhash{#1}{-45}$\cr
		$#1\xxhash{#1}{45}$\cr
	}%
}
\newcommand{\xxhash}[2]{\rotatebox[origin=c]{#2}{$#1\parallel$}}

% circled relations
\makeatletter
\newcommand{\ogeneric}[2][0.7]{%
	\vphantom{\oplus}\mathpalette\o@generic{{#1}{#2}}%
}
\newcommand{\o@generic}[2]{\o@@generic#1#2}
\newcommand{\o@@generic}[3]{%
	\begingroup
	\sbox\z@{$\m@th#1\oplus$}%
	\dimen@=\dimexpr\ht\z@+\dp\z@\relax
	\savebox\tw@[\totalheight]{$\m@th#1\bigcirc$}%
	\makebox[\wd\z@]{%
		\ooalign{%
			$#1\vcenter{\hbox{\resizebox{\dimen@}{!}{\usebox\tw@}}}$\cr
			\hidewidth
			$#1\vcenter{\hbox{\resizebox{#2\dimen@}{!}{$#1\vphantom{\oplus}{#3}$}}}$%
			\hidewidth
			\cr
		}%
	}%
	\endgroup
}
\makeatother

\newcommand{\ole}{\mathrel{\ogeneric{<}}}
\newcommand{\oleq}{\mathrel{\ogeneric[0.6]{\leq}}}
\newcommand{\oprec}{\mathrel{\ogeneric[0.6]{\prec}}}
\newcommand{\opreceq}{\mathrel{\ogeneric[0.6]{\preceq}}}
\newcommand{\oaste}{\mathbin{\ogeneric[0.6]{\ast}}}
\newcommand{\oneg}{\mathrel{\ogeneric[0.6]{\underline{\neg}}}}
\newcommand{\oefunc}{\mathrel{\ogeneric[0.6]{e}}}
\newcommand{\oewedge}{\mathrel{\ogeneric[0.6]{\underline{\wedge}}}}
\newcommand{\osucc}{\mathrel{\ogeneric[0.6]{\mathsf{S}_a}}}

%% End of Personal Macros %%%
